Intrinsic Robustness of Prophet Inequality to Strategic Reward Signaling

Prophet inequality concerns a basic optimal stopping problem and states that simple threshold stopping policies -- i.e., accepting the first reward larger than a certain threshold -- can achieve tight $\frac{1}{2}$-approximation to the optimal prophet value. Motivated by its economic applications, this paper studies the robustness of this approximation to natural strategic manipulations in which each random reward is associated with a self-interested player who may selectively reveal his realized reward to the searcher in order to maximize his probability of being selected. We say a threshold policy is $\alpha$(-strategically)-robust if it (a) achieves the $\alpha$-approximation to the prophet value for strategic players; and (b) meanwhile remains a $\frac{1}{2}$-approximation in the standard non-strategic setting. Starting with a characterization of each player's optimal information revealing strategy, we demonstrate the intrinsic robustness of prophet inequalities to strategic reward signaling through the following results: (1) for arbitrary reward distributions, there is a threshold policy that is $\frac{1-\frac{1}{e}}{2}$-robust, and this ratio is tight; (2) for i.i.d. reward distributions, there is a threshold policy that is $\frac{1}{2}$-robust, which is tight for the setting; and (3) for log-concave (but non-identical) reward distributions, the $\frac{1}{2}$-robustness can also be achieved under certain regularity assumptions.

==> arXiv/1-intro.tex <==

\newcommand{\prophet}{\cc{OPT}}

Prophet inequality stands out as a key result in optimal stopping theory, addressing the optimal timing for decision-making to maximize the expected reward.
In the classic setting, a searcher faces a finite sequence of $\boxNum$ boxes each containing non-negative random reward $X_i$. For every $i \in [\boxNum]$, box $i$'s reward $X_i$ is drawn from known distribution $\prior_i$. $(\prior_i)_{i \in [\boxNum]}$ are assumed to be independent. While the searcher knows each box's reward distribution, the actual realization of the reward $X_i\sim\prior_i$ for $i\in[\boxNum]$
are revealed iteratively.
Upon seeing a reward, the searcher can either accept the reward and the game ends, or reject the reward and the next reward is presented to her.
The searcher aims to design a stopping policy that maximizes her expected payoff. It's clear that the searcher's expected payoff cannot exceed $\E[\max_{i \in [\boxNum]} X_i]$. This is exactly the expected payoff of a prophet who can see in advance the realizations of all the random rewards. A seminal result by \cite{KS-78} showed that there exist a stopping policy that can guarantee the searcher at least half of $\E[\max_{i \in [\boxNum]} X_i]$ as reward. Such a result, that gives a stopping policy whose expected reward is comparable to $\E[\max_{i \in [\boxNum]} X_i]$, is called a prophet inequality.

Remarkably, \cite{KS-78,KUS-77} also showed that 
there exist very elegant threshold stopping policies
that guarantees the searcher at least $\sfrac{1}{2}$ of $\E[\max_{i \in [\boxNum]} X_i]$, and this constant of $\sfrac{1}{2}$ is tight. A threshold stopping policy is a policy where the searcher pre-computes a value $T$ as a function of $(\prior_i)_{i \in [\boxNum]}$, and accepts the first reward that is no less than $T$. Subsequent contributions by \citep{KW-12,SC-84} established a spectrum of thresholds, within which any threshold stopping policy is optimal, showcasing versatility of prophet inequalities. 

An important assumption in the classic prophet inequality is that each box is an inanimate object and, once the searcher reaches it, will fully disclose its realized reward to the searcher. Yet this may not be the case in many real-world applications where boxes often correspond to real strategic players who may have incentives to selectively disclose information to maximize their own probability of being chosen by the searcher. This is usually the case when information is not controlled by nature but by humans or algorithms. Consider the following two examples.

\rz{two examples need to be modified: both examples mention commitment, this needs to be changed}
\begin{example}[Online Advertising]
In online advertising, the platform (searcher) commits to a searching policy, determining how it selects and displays ads to users based on their search queries. Such a searching policy may consider factors like bid amount, relevance, and historical user behavior to determine which ads to display. Advertisers are presented to the searcher iteratively. Each advertiser bids for the opportunity to have their ads displayed when users make relevant search queries. In the classic setting, each advertiser truthfully reveal full information regarding their bid amount and relevance. However, in real world, advertisers can strategically deviate from their initial bid amounts or relevance to influence their ad's likelihood of being displayed. The goal of the searcher is to design a stopping policy that selects an advertiser and maximizes user engagement. Our work studies the searcher's optimal stopping policy when she knows that advertisers are strategically revealing information.
\end{example}

\begin{example}[Accepting Job Offers]
A job seeker (searcher) receives job offers in a rolling basis and commits to a searching policy, determining how she chooses to accept an offer. Such a searching policy may involve criteria such as company reputation, initial salary and expected growth, and benefits. Job offers are presented to the searcher iteratively with one-day exploding offers; the seeker must accept or reject the offer immediately. Each offer specifies details such as job requirements, responsibilities, and compensation. In the classic setting, employer truthfully reveal such details. However, employers can strategically deviate from their details to increase their chances of being accepted by the candidate. The goal of the searcher is to design a stopping policy that selects the best job for her to accept. This paper studies the job seeker's optimal stopping policy when she knows that employers are strategically revealing job details to increase the seeker's probability to sign the offer letter. 
\end{example}

Motivated by the above real-world applications, we consider a natural variant of the prophet inequality problem where each box is associated with a strategic player. Due to the elegance and simplicity nature of threshold stopping policies, the focus of this paper is to investigate the intrinsic robustness of these threshold stopping policies to strategic information revelation. More precisely, we aim to understand which threshold within the known $\sfrac{1}{2}$-approximation spectrum can give rise to threshold stopping policy that guarantees the searcher payoff that is comparable to $\E[\max_{i \in [\boxNum]} X_i]$ in both the classic(non-strategic) setting and strategic setting. 



%We model this as a multi-player Stackelberg game where the searcher first commits to a stopping policy, and then, each box designs his information revealing strategy to maximizes his own probability of being chosen by the searcher. In this setting, the searcher's stopping policy can depend on both boxes' priors $(\prior_i)_{i\in[\boxNum]} $ and boxes' information revealing strategies. Knowing that the boxes will best respond to her searching strategy, the searcher wants to design a stopping policy that will maximize her expected payoff. We formalize the setting in \Cref{sec:setting}. 

%Similar to the classic setting, the searcher's payoff can be no more than that of the prophet who is clairvoyant and can see in advance the realization of all the random variables. As we show later in \Cref{sec:classic}, a good stopping policy in the classic setting might perform bad in the strategic environment, and vice versa. The focus of this paper is to design informationally robust stopping policies for the searcher such that it performs well in both the classic setting where boxes are not being strategic and in the setting that we introduced where each box is associated with a strategic sender who can design his own information revealing strategy.

\subsection{Our Contributions}

We now describe our results in more detail.

\xhdr{Optimal Information Revelation} In the strategic setting, each player want to best respond to the searching policy that the searcher announces. We show in \cref{sec:opt infor} that when the searcher uses a threshold stopping policy (\cref{defn:threshold}), each player’s optimal information revealing strategy can be well-characterized (\cref{prop:optimal signaling scheme}). Intuitively, since the threshold $T$ that the searcher pre-computes is independent of the information revealing strategy each player uses, each player want to use a strategy that gives her the highest probability of beating the threshold $T$. As a corollary of \cref{prop:optimal signaling scheme}, the interaction between the searcher and the player can be simplified: 
(1) The searcher first decides a stopping threshold $T$.
(2) Each player $i$ chooses the distribution $G_i$ defined as in \Cref{prop:optimal signaling scheme} according to his prior 
$\prior_i$ and the threshold $T$.
(3) The searcher visits each $G_i$ sequentially and stops when the first realized reward $X_i\ge T$ 
where $X_i\sim G_i$.

With the above game timeline, we can formally define what it means for a stopping policy to be $\alpha$-robust. Let $u(T;\prior_{1:\boxNum})$ denote the expected payoff of the searcher when she uses threshold stopping policy with threshold $T$ against players that play distributions $\prior_{1:\boxNum}$, and let $\prophet \triangleq \expect[X_i \sim \prior_i]{\max_{i\in[\boxNum]}X_i}$. We say a threshold stopping policy with threshold $T$ is $\alpha$-robust if both $u(T;\prior_{1:\boxNum}) \ge \alpha \cdot \prophet$ and $u(T;G_{1:\boxNum}) \ge \alpha \cdot \prophet$ hold. 
 
\xhdr{Robust Policy for General Distributions} Our first main results shows that there exist threshold within the $\sfrac{1}{2}$-approximation spectrum that is $\frac{1-\sfrac{1}{e}}{2}$-robust for all general distributions (\cref{thm:general prior}). Moreover, this ratio of $\frac{1-\sfrac{1}{e}}{2}$ is also tight in the sense that no other threshold within the known $\sfrac{1}{2}$-approximation spectrum can guarantee better approximation ratio. Note that this does not exclude the fact there there could exist some threshold outside of the $\sfrac{1}{2}$-approximation spectrum that can beat the ratio of $\frac{1-\sfrac{1}{e}}{2}$. Since it's outside of the spectrum of the paper, we won't investigate further. \rz{however, we do have the $1/2$ approximation dynamic threshold policy under deviation result.}


\xhdr{Robust Policy for Special Distributions} Our next two main results establishes $\sfrac{1}{2}$-robust threshold stopping policy for two classes of distributions: (1) Independent and identically distributed priors $\prior \equiv \prior_i$ for all $i\in[\boxNum]$  (\cref{thm:IID prior}); (2) Log-concave heterogeneous distributions (\cref{thm:mainOblivious}).

\begin{comment}
Summary of our current results:
\begin{itemize}
    \item We fully characterize the Stackelberg equilibrium for $2$ boxes given 
    various searcher's searching policies: 
    (1) fixed-threshold policy that only depends on 
    boxes' priors (include \OPT);
    (2) threshold policy that could depend on 
    boxes' information strategies (include \HEM, \MEDIAN);
    \item 
    Fix an searcher's searching policy, 
    we compare searcher's payoff when boxes are not allowed
    to strategically reveal reward information and when 
    boxes are allowed
    to strategically reveal reward information (under $2$ boxes);
    \item 
    We study searcher's problem and fully  
    characterize searcher's optimal searching policy when the boxes can strategically reveal reward information (generalized to $N$ boxes)
\end{itemize}
\end{comment}

%Our contributions are three-fold: (1) we characterize the searcher's optimal stopping policies in our setting; (2) we formally define informationally robust $\alpha$-approximation policies, and provide characterization of a robust policy that guarantees the searcher at least half of the prophet's payoff under some mild assumptions on the boxes' priors; and (3) we characterize the Stackelberg equilibrium when the searcher uses classic policies under the two-box setting and show that the searcher's payoffs under these equilibria are suboptimal.

%We first categorize the searcher's policies into three classes: \textit{general stopping policies} which can depend on both of the boxes' priors and signaling schemes, \textit{posterior-free stopping policies} which only depend on the boxes' priors, and \textit{prior-free stopping policies} which only depend on the boxes' signaling schemes. We show that when the searcher uses a posterior-free stopping policy or a prior-free stopping policy, the boxes signaling schemes can be effectively reduced to  distributions over posterior means which can be characterized by mean-preserving spread.

%The benchmark that we compare the searcher's expected reward with is $\OPT = \E[\max_{i \in [\boxNum]} X_i]$, the expected reward of the prophet who is clairvoyant and can see in advance the realizations of all random variables. We show in \ref{claim:lowerBound} that no policy can guarantee strictly more than half of the prophet's payoff, so the best approximation ratio we can hope for is $\sfrac{1}{2}$.

%We now describe each of our contributions in detail.


%\xhdr{Optimal Searching Policies} We first show that there exist a general stopping policy for the searcher where she essentially forces the boxes to always reveal full information: the searcher threatens the boxes by automatically rejecting their reward if they deviate away from the priors. The searcher can then use any $\sfrac{1}{2}$-approximation policy in the classic setting to get $\sfrac{1}{2}$-approximation in the setting where boxes are allowed to be strategic. This observation motivates us to look into posterior-free stopping policies and prior-free stopping policies.

%In the literature of prophet inequalities, all classic policies are threshold policies where the searcher accepts the reward if the reward exceeds her set threshold for each box. The searcher sets threshold $T_i$ for each box $i$ and she stops searching and accepts $X_i$ only when $X_i \ge T_i$. The main result we have is that there exist a posterior-free threshold policy for the searcher where she can obtain optimal payoff in the setting that we introduced. We first show that when the searcher uses a posterior-free threshold policy, the boxes' best response strategies are deviating to "binary pooling" strategies where their upper supports are equal to the thresholds $T_i$, since this maximizes the probabilities they realize a reward $X_i \ge T_i$. The searcher can then strategically assign $T_i$ such that when the boxes play their best response strategies, the searcher achieves the same payoff as the optimal payoff under no deviation which is given by the dynamic programming policy. We also prove that this is the optimal payoff under any posterior-free policy, using properties of second-order stochastic dominance.

%\xhdr{Robust Searching Policies} We say a searching policy is a robust $\alpha$-approximation policy if the searcher's payoff exceeds $\alpha$ fraction of \OPT\ both in the classic setting and in the setting where boxes can be strategic. Since $\alpha = \sfrac{1}{2}$ is the best approximation ratio we can hope for, we attempt to find robust $\sfrac{1}{2}$-approximation policies. 

%Our main result is showing the existence of robust searching policies when there are many boxes with log-concave truncated distributions. We care about this family of distributions because they include a lot of common distributions such as Gaussian, Chi-Squared, Beta, Exponential, etc. We prove this by showing that the cumulative distribution function, $\Bar{\prior}$, of the max of the boxes' rewards under no deviation is convex, and with the observation that the mean is less than the median for a convex function, we show that a simple threshold posterior-free policy where the searcher uses any threshold between the mean and the median of $\Bar{\prior}$ is a robust $\sfrac{1}{2}$-approximation policy.

%\xhdr{Classic Searching Policies} Lastly, we analyze the performance of known classic policies where the searcher achieves $\sfrac{1}{2}$ of the prophet's value under no deviation, namely \DP-H, the dynamic threshold policy achieving optimal payoff, \HEM-H, a simple threshold policy where the searcher accepts any reward greater than $\sfrac{1}{2}$ of the prophet's value, and \MEDIAN-H, a simple threshold policy where the searcher accepts any reward greater than the median of the max of the boxes' rewards. In our paper, we define \DP, \HEM, and \MEDIAN\ as the prior-free versions of these policies, where the searcher computes the thresholds based off of the signaling schemes $G$ of the boxes.  

%We first characterize the boxes' Stackelberg Equilibria for these prior-free policies when there are only two boxes. In all of these cases we prove that box $1$ deviates to a binary pooling strategy. \DP\ has a simple solution since box $1$ just needs to exceed the mean of box $2$, \HEM\ requires box $2$ to reveal full information to increase the threshold for box $1$ to pass due to the convexity of the \HEM\ threshold, and \MEDIAN\ requires box $2$ to use a specific binary pooling policy to increase the threshold for box $1$ to pass.

%We then show through some counterexamples that none of these policies achieve $\sfrac{1}{2}$ of \OPT\ for the searcher. Finally, we analyze whether the posterior-free policies \DP-H, \HEM-H, and \MEDIAN-H, achieve $\sfrac{1}{2}$ of \OPT\ when the boxes optimally deviate, which would show that these policies are $\sfrac{1}{2}$-robust. We show through some counterexamples that none of these policies achieve this result.









==> arXiv/apx-classic.tex <==

\label{sec:classic}
\newcommand{\interimMaxPrize}{v}


\newcommand{\cutoff}{t}
\newcommand{\cutoffInfor}{G^{(t)}}
\newcommand{\equilCutoff}{t^*}

\newcommand{\remainMaxMean}{\bar{\priorMean}}




As we can see from above definition, 
the \DP\ policy sets different thresholds when reaching 
to different  random variables. 
A classic result of \cite{KUS-77,KS-78} states that,
by using a fixed-threshold policy that accepts the
first reward that is no smaller than this threshold,
the searcher
can obtain at least half of the expected reward that a prophet can make who knows the realizations of the rewards beforehand.
% set by the \DP\ policy are computed by 
% via the dynamic program, which could be generally computationally intractable due to the  
% Given the boxes' garbled strategies $G$, the OPT policy is well-known to be optimal for the searcher's payoff. There are other policies for the searcher to consider, namely those that give $1/2$-approximations to the optimal one.
% \begin{definition} [threshold policy]
%     \item A \textit{strict threshold policy} is a policy where the searcher will claim the first signalled reward larger than a threshold. Similarly, a \textit{non-strict threshold policy} is a policy where the searcher claims the first signalled reward larger than or equal to a threshold.
% \end{definition}
% We will also consider the Half-Expected-Max and Median policies in our paper since they are known to be $1/2$-approximations of the optimal policy. 
Indeed, there are different thresholds that can 
guarantee such half approximation. 
In this work, we focus on two such threshold policies:
\begin{definition}[\HEM\ stopping policy]
Given a sequence of distributions $\prior_1, \cdots, \prior_\boxNum$, 
a Half-Expected-Max policy (henceforth \HEM) is a 
threshold policy where the searcher accepts the first reward 
whose value is larger than or equal to $\sfrac{1}{2} \expect{\max\{X_1, \ldots, X_\boxNum\}}$.
\end{definition}
% Given a strategy profile $(G_1, \ldots,G_\boxNum)$, we use  
% \[\HEMthreshold(G_1, \ldots,G_\boxNum) \triangleq \sfrac{1}{2} \expect[\maxPrize\sim \maxPrizeCDF]{\maxPrize}\] 
% to denote the resulting threshold where the searcher will accept the first reward 
% whose value exceeds this threshold under the policy.

% Other than using the half-expected-max as the threshold, 
% there also exists other fixed-threshold policy that can also 



\begin{definition}[\MEDIAN\ stopping policy]
\label{Med_defn}
Given a sequence of distributions $\prior_1, \cdots, \prior_\boxNum$, 
a Median policy (henceforth \MEDIAN)
is a threshold policy where the searcher accepts the first reward whose value is larger than or equal to $\inf\{c: \prob{\max\{X_1, \ldots, X_\boxNum\} \ge c} \le \sfrac{1}{2}\}$.
\end{definition}

We first analyze the application of these stopping policies to the prior-free setting, where the boxes first reveal their signaling schemes $G_i$ to the searcher and she computes the thresholds based off of them, setting $\prior_i = G_i$ in the above definitions. We first show the Stackelberg Equilibria solutions for these policies when there are two boxes, where the boxes deviate to the strategies $G_i$ that maximize their own individual payoffs.

To be precise, the \MEDIAN\ stopping policy for the priors is a $\sfrac{1}{2}$-approximation, since by our assumption they are continuous. In the new setting, it is possible for the boxes to deviate to non-continuous strategies $G_i$, such that the searcher does not even achieve $\sfrac{1}{2}$-approximation if the $G_i$s were the true priors. However, this is an irrelevant concern because the $\sfrac{1}{2}$ benchmark we are comparing to is set by the priors $\prior_i$.

\subsection{Analyzing Boxes' Stackelberg Equilibrium}
We first show the Stackelberg Equilibria solutions for the \DP, \HEM, and \MEDIAN\ stopping policies in the two-box setting.

In some of the following equilibria slutions, the first box can use the no-information strategy and always get selected. An observation is that if this is possible, any other strategy for the first box maximizing their own payoff gives the searcher the same expected reward, which is $\priorMean_1$. 

The following are the main results of our section:

\begin{theorem}[Stackelberg equilibrium for two-box under \DP]
\label{prop: stackelberg dp}

    Consider a two-box setting $N = 2$, and arbitrary priors $\prior_1, \prior_2$. If the searcher uses the OPT policy, then for any $G_2\blackwellOrder \prior_2$:
    \begin{itemize}
        \item when $\priorMean_1 \ge \priorMean_2$, 
        then $(\noInfor(\priorMean_1), G_2)$ forms 
        an equilibrium;
        \item when $\priorMean_1 < \priorMean_2$, 
        then $(G^{(t^*)}, G_2)$ forms 
        an equilibrium where $G^{t^*}$ is a binary pooling strategy
        with the cutoff $t^*$ satisfying $\expect[x\sim G^{t^*}]{x \mid x\ge t^*} = \priorMean_2$.
        % then box $1$ should use a binary pooling strategy with $b_1 = \priorMean_2$, and box $2$'s strategy doesn't matter.
    \end{itemize}
\end{theorem}

\begin{theorem}[Stackelberg equilibrium for two-box under \HEM]
\label{prop: stackelberg hem}
Consider a two-box setting $\boxNum = 2$, 
and arbitrary priors $\prior_1, \prior_2$. 
% but with the same mean $\priorMean_1 = \priorMean_2 \equiv \priorMean$.
When the searcher uses \HEM,
there exists a binary pooling strategy $\equilStrat \equiv G^{(t^*)}$ with the cutoff $t^*$
such that $(\equilStrat, \prior_2)$ forms an equilibrium. 
Let function $\interimMaxPrize_1(x) = \expect[x_2\sim \prior_2]{\max\{x, x_2\}}$ for $x \in [0,1]$.
Then equilibrium strategy $\equilStrat$ with support 
$\supp(\equilStrat) = \{a(\equilCutoff), b(\equilCutoff)\}$
satisfies  
\begin{itemize}
    \item when $\priorMean_1 \ge \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$, 
    box $1$ should use the no-information strategy;
    \item when $\priorMean_1 < \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$, 
    there exists a unique $\equilCutoff$ such that $b(\equilCutoff) = \HEMthreshold(\equilStrat, \prior_2)$.
    % $\equilCutoff$ is the root of the function 
    % $f(\cutoff) = \thres(\cutoffInfor, \prior_2) - b(\cutoff)$.
\end{itemize}
\end{theorem}

\begin{theorem}[Stackelberg equilibrium for two-box under \MEDIAN]
\label{prop: stackelberg median}
    Consider a two-box setting $N = 2$, and arbitrary priors $\prior_1,\prior_2$. If the searcher uses the \MEDIAN\ policy, then for some threshold $\BM$ computed by the priors:
    \begin{itemize}
        \item when $\priorMean_1 \ge \BM$, box $1$ always wins by sending the no information strategy.
        \item when $\priorMean_1 < \BM$, then the Stackelberg equilibrium $(G_1^{*},G_2^{*})$ consists of box $1$ using the binary pooling strategy with $b_1 = \BM$, and box $2$ using the binary pooling strategy with $b_2 = \BM$.
    \end{itemize}
\end{theorem}

We first prove the Stackelberg equilibrium for the \DP\ setting.

\subsubsection{Proof of \DP\ Stackelberg Equilibrium}

We notice that when the searcher uses \DP\ policy, 
no matter which  information strategy the box $2$ is using,
the searcher claims prize from box $1$ if and only if the realized 
prize from box $1$ is no smaller than $\priorMean_2$. Thus, by \Cref{constant threshold policy multibox}, setting $T_1 = \priorMean_2$, when $\priorMean_1\ge T_1$, box $1$ can maximize its payoff using the no-information strategy, and when $\priorMean_1<T_1$, using the binary pooling strategy 
$\equilStrat_1$ with support $\supp(\equilStrat_1) = \{a, T_1\}$
maximizes box $1$'s probability on realizing a prize no smaller than $T_1$. 

We now sketch the steps to prove the Stackelberg equilibria for the \HEM\ and \MEDIAN\ settings, and the details of the proofs are deferred to Appendix \ref{sec:appendix}.

\subsubsection{Proof of \HEM\ Stackelberg Equilibrium}

We prove \Cref{prop: stackelberg hem} with following steps: 
\begin{enumerate}
    \item We first show that it is always (weakly) better 
    for box $2$ to use full information
    strategy no matter what priors $\prior_1, \prior_2$ are 
    (see \Cref{prop: last box behavior});
    \item When $\priorMean_1 \ge \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$, 
    no information strategy is 
    the best-response strategy for box $1$ (see \Cref{equilibrium case 1});
    \item When $\priorMean_1 < \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$,
    \begin{enumerate}
        \item 
        We show that box $1$ always prefers a strategy $G$ with binary support $\supp(G) = \{a, b\}$
        (see \Cref{binary-supp suffices});
        \item 
        We then show that there always exists a best-response strategy for box $1$ that is a binary pooling strategy (see \Cref{cutoff infor suffices});
        \item We then show that the equilibrium binary pooling strategy
        $\equilStrat \equiv G^{(\equilCutoff)}$ must satisfy that 
        $b(\equilCutoff) = \HEMthreshold(\equilStrat, \prior_2)$ and 
        such $\equilCutoff$ always exists (see \Cref{lem:existence of equilCutoff}). 
        \item Lastly, we show that this $\equilCutoff$ is unique. (see \Cref{uniqueness of $\equilCutoff$})
    \end{enumerate}
\end{enumerate}

\subsubsection{Proof of \MEDIAN\ Stackelberg Equilibrium}

We prove \Cref{prop: stackelberg median} with following steps: 
\begin{enumerate}
    \item We first show that box $2$ always prefers a strategy $G_2$ with binary support (see \Cref{median support 2} and \Cref{median pooling 2})
    \item when $\priorMean_1 \ge \BM$, box $1$ always wins by sending the no information strategy. (see \Cref{no info wins})
    \item when $\priorMean_1 < \BM$, then the Stackelberg equilibrium $(G_1^{*},G_2^{*})$ consists of box $1$ using the binary pooling strategy with $b_1 = \BM$, and box $2$ using the binary pooling strategy with $b_2 = \BM$. (see \Cref{stackelberg exists})
\end{enumerate}



\subsection{Half Expected Reward Doesn't Hold}
We saw previously that the searcher's optimal stopping policy under deviation achieves the same expected payoff as the optimal stopping policy in the no deviation case, which is known to be a $\sfrac{1}{2}$-approximation. Under no deviation, \DP, \HEM, and \MEDIAN\ are often widely used because they achieve $\sfrac{1}{2}$-approximation. In this section, we will construct examples to show that the searcher does not achieve $\sfrac{1}{2}$-approximation under these policies when the boxes can deviate.

\begin{proposition}
    \HEM\ is not a $\sfrac{1}{2}$-approximation under deviation.
\end{proposition}

\begin{proof}
    Consider the scenario where there are two boxes with priors $\prior_1$ and $\prior_2$, uniformly distributed on $[0,0.5]$ and $[0,0.92]$ respectively. Note $\priorMean_1 = 0.25$ and $\priorMean_2 = 0.46$.

    We first compare $\priorMean_1$ to $\interimMaxPrize_1(\priorMean_1)$. The latter value is $\expect[h_2 \in \prior_2]{\max\{\priorMean_1, h_2\}}$, and can be computed as 
    \begin{align*}
       \interimMaxPrize_1(\priorMean_1) = \frac{0.25}{0.92} \times 0.25 + (1-\frac{0.25}{0.92}) \times \frac{0.25+0.92}{2} \approx 0.4940
    \end{align*}
    By \Cref{prop: stackelberg hem}, box $1$ should play the no-information strategy $\delta(G_1)$, in which case the searcher's payoff is $\priorMean_1 = 0.25$. But the prophet reward is 
    \begin{align*}
        \expect{\max\{X_1, X_2\}} = \frac{0.5}{0.92} \times \frac{1}{3} + (1-\frac{0.5}{0.92}) \times \frac{0.5 + 0.92}{2} \approx 0.5053
    \end{align*}
    Hence, we can see the searcher's payoff is $< \expect{\max\{X_1, X_2\}}/2$, which means that they do not achieve a $\sfrac{1}{2}$-approximation.
\end{proof}

\begin{comment}
\begin{lemma}
    \DP\ is a $\sfrac{1}{2}$-approximation under deviation when there are only two boxes.
\end{lemma}

\begin{proof}
    From \Cref{prop: stackelberg dp}, box $1$ sets $b_1 = \max\{\priorMean_1,\priorMean_2\}$, and the searcher's payoff is actually $\max\{\priorMean_1,\priorMean_2\}$. By \Cref{lemma: bounding HEM}, we see that this value is $\ge \frac{\priorMean_1+\priorMean_2}{2} \ge \expect{\max\{X_1, X_2\}}/2$, so the searcher achieves $\sfrac{1}{2}$-approximation.
\end{proof}
\end{comment}

\begin{comment}
\begin{lemma}
    \MEDIAN\ is a $\sfrac{1}{2}$-approximation under deviation when there are only two boxes.
\end{lemma}

\begin{proof}
    We can see from \Cref{prop: stackelberg median}, box $1$ sets $b_1 = \max\{\priorMean_1,\BM\}$. If $\priorMean_1 \ge \BM$, then $\priorMean_1 \ge \priorMean_2$ as well, and the searcher always accepts box $1$ so their payoff will be $\priorMean_1 \ge \expect{\max\{X_1, X_2\}}/2$ by \Cref{lemma: bounding HEM}. If $\priorMean_1 < \priorMean_2$, then box $1$ sets $b_1 = \BM$, and the searcher's payoff will be a linear combination of $\priorMean_2$ and $\BM \ge \priorMean_2$, which is at least $\priorMean_2 \ge \expect{\max\{X_1, X_2\}}/2$.

    Finally, we examine the case where $\priorMean_2 \le \priorMean_1 \le \BM$. Note that $\BM \le 2\priorMean_2$, since $\BM$ is a support of mass $\frac{1}{2}$ in a binary pooling distribution with mean $\priorMean_2$. Then $\expect{\max\{X_1, X_2\}} \le \priorMean_1 + \priorMean_2 \le 3\priorMean_2$. \dz{Incorrect...} But the searcher's payoff is a linear combination of $\priorMean_2$ and $\BM \ge \priorMean_2$, which is at least $\priorMean_2$. no conclusion
\end{proof}
\end{comment}


\begin{proposition}
    \DP\ is not a $\sfrac{1}{2}$-approximation under deviation.
\end{proposition}

\begin{proof}
    Consider the scenario where there are three boxes with priors $H_1,H_2,H_3$, such that $H_1$ has a singular mass support on $\priorMean_1 = 0.2$ and $H_2,H_3$ are on support $\{0,1\}$ with $\priorMean_2 = \priorMean_3 = 0.25$.

    Under the \DP\ policy, box $1$ will never get selected by the searcher, because they can only offer a reward of $0.2$ which is always going to be worse than if the searcher rejects them. This is because once the searcher rejects box $1$, their expected payoff is at least $0.25$, or the expected reward of the third box, since under \DP, the searcher will not implement a policy where their expected payoff is worse than rejecting the first $(\boxNum-1)$ boxes.

    Thus, our game reduces to a two boxes, where by \Cref{prop: stackelberg dp}, the searcher's payoff is $\max\{\priorMean_2,\priorMean_3\} = 0.25$. But we also compute 
    \begin{align*}
        \expect{\max\{X_1, X_2,X_3\}} = (1-0.25)^2 \times 0.2 + (1-(1-0.25)^2) \times 1 = 0.55 
    \end{align*}
    Since $0.55/2 > 0.25$, the searcher does not achieve a $\sfrac{1}{2}$-approximation under \DP.
\end{proof}

\begin{proposition}
    \MEDIAN\ is not a $\sfrac{1}{2}$-approximation under deviation.
\end{proposition}

\begin{proof}
    Consider the scenario where there are three boxes with priors $H_1,H_2,H_3$, such that $H_1$ has a singular mass support on $\priorMean_1 = 0.39$ and $H_2,H_3$ are on support $\{0,1\}$ with $\priorMean_2 = \priorMean_3 = 0.2$.

    Under the \MEDIAN\ policy, box $1$ will never get selected by the searcher. This is because the latter two boxes, by \Cref{prop: stackelberg median}, play binary pooling strategies with $b_2 = b_3 = \BM = 0.4$, and under this strategy profile, box $1$ is not chosen because $\bar{G}(0.2) = 1 \cdot 0.5 \cdot 0.5 < 0.5$. Since box $1$ cannot deviate, no box under this strategy profile can deviate to a more profitable strategy, so this is the Stackelberg Equilibrium with all three boxes included as well.

    Under this strategy profile, since the support $b_2$ has probability mass $1/2$ and box $1$ never gets selected, the searcher's payoff is 
    \begin{align*}
        0.5 \times 0.4 + (1-0.5) \times 0.2 = 0.3.
    \end{align*}

    We can also compute 
    \begin{align*}
        \expect{\max\{X_1, X_2,X_3\}} = (1-0.2)^2 \times 0.39 + (1-(1-0.2)^2) \times 1 = 0.6096
    \end{align*}
    Since $0.6096/2 > 0.3$, the searcher's payoff under the \MEDIAN\ policy in this setting is not a $\sfrac{1}{2}$-approximation.
\end{proof}

\subsection{Classic Policies Not Information Robust}

Another question to ask is if \DP, \HEM, and \MEDIAN\ under no deviation are informationally robust; that is, if the boxes deviate to their best responses, does the searcher still achieve a $\sfrac{1}{2}$-approximation? If she does then this shows that the searcher can use a much simpler policy than the ones described in earlier sections to achieve a good payoff. We show in this section that the answer to this question is no. To avoid confusion, we will call these policies \DP-H, \HEM-H, and \MEDIAN-H. Note these policies are independent of the boxes' deviation strategies; hence they are posterior-free policies.

Since these policies $q$ are all of the form $q_i = \indicator{x \ge T_i}$, since the searcher can precompute all of the thresholds $T_i$ assuming the boxes play their priors, we know from \Cref{constant threshold policy multibox} that the boxes should deviate to binary pooling strategies setting $b_i = \max\{T_i,\priorMean_i\}$.

\subsubsection{Two-Box Setting}

Our results show that while \MEDIAN-H\ is not a $\sfrac{1}{2}$-approximation, \DP-H\ and \HEM-H\ are indeed $\sfrac{1}{2}$-approximations under deviation when there are only two boxes. This also implies that \DP-H\ and \HEM-H\ are robust $\sfrac{1}{2}$-approximation policies for the two-box setting. 

We first prove a useful lemma in the two-box setting.

\begin{lemma}
\label{lemma: bounding HEM}
$\HEMthreshold(\prior_1,\prior_2) \le \frac{\priorMean_1+\priorMean_2}{2}$
\end{lemma}
\begin{proof}
    Recall that $\interimMaxPrize_1(x) = \expect[x_2\sim \prior_2]{\max\{x, x_2\}}$ for $x \in [0,1]$. We have
\begin{align*}
    \HEMthreshold(\prior_1,\prior_2) 
    &= \frac{1}{2} \expect[x\sim \prior_1]{\expect[x_2\sim \prior_2]{\max\{x, x_2\}}} 
    = \frac{1}{2}\int_0^1  \interimMaxPrize_1(x) \ \mathrm{d}\prior_1(x)\\
    &= \frac{1}{2}\int_0^1   \big(\expect[y\sim \prior_2]{y\mid y\ge x} \cdot \prob[y\sim \prior_2]{y \ge x}  + x 
    \cdot \prob[y\sim \prior_2]{y < x}\big) \ \mathrm{d}\prior_1(x) \\ 
    &\le \frac{1}{2}\int_0^1  (\priorMean_2 + x) \ \mathrm{d}\prior_1(x) 
    \le \frac{1}{2}\Big(\int_0^1  x \ \mathrm{d}\prior_1(x) + \priorMean_2\Big)
    = \frac{\priorMean_1+\priorMean_2}{2}
\end{align*}
\end{proof}

\begin{proposition}
    \MEDIAN-H is not a $\sfrac{1}{2}$-approximation under deviation.
\end{proposition}

\begin{proof}
    Consider the example where $\prior_1$ is uniform on $[0,\frac{1}{24}]$ with weight $\frac{5}{6}$ and uniform on $[\frac{23}{24},1]$ with weight $\frac{1}{6}$, and $\prior_2$ is uniform on $[0,\frac{1}{24}]$ with weight $\frac{3}{5}$ and uniform on $[\frac{23}{24},1]$ with weight $\frac{2}{5}$. We can compute $\priorMean_1 = \frac{13}{72}$ and $\priorMean_2 = \frac{97}{240}$.

    The \MEDIAN-H\ threshold is $\frac{1}{24}$, since $\overline{\prior}(\frac{1}{24}) = \prior_1(\frac{1}{24})\prior_2(\frac{1}{24}) = \frac{5}{6} \times \frac{3}{5} = \frac{1}{2}$, and there is no $x < \frac{1}{24}$ where $\overline{\prior}(x) \ge \frac{1}{2}$. Thus, box $1$ should deviate to $\delta(\priorMean_1)$, since $\frac{13}{72} > \frac{1}{24}$. The searcher's payoff is then $\priorMean_1 = \frac{13}{72}$.

    %Unlike the \HEM\ threshold under no deviation, we also need to check that under no deviation, this specific \MEDIAN\ threshold $T = \frac{1}{24}$ indeed is part of the well-known spectra of $1/2$-approximation strategies. This requires $T \le \mathbb{E}[(c_1-T)_+] + \mathbb{E}[(c_1-T)_+]$, where $c_i$ is the expected reward the searcher gets from box $i$.  Note the RHS is $\frac{1}{6} \cdot (\frac{47}{48} - \frac{1}{24}) + \frac{2}{5} \cdot (\frac{48}{48} - \frac{1}{24}) = \frac{17}{32} \ge \frac{1}{24}$. 

    We can also compute $\expect[X_i \sim \prior_i] {\max\{X_i\}} = \frac{\frac{5}{6} \times \frac{3}{5} \times \frac{1}{36} + \frac{5}{6} \times \frac{2}{5} \times \frac{47}{48} + \frac{1}{6} \times \frac{3}{5} \times \frac{47}{48} + \frac{1}{6} \times \frac{2}{5} \times \frac{71}{72}}{2} \approx 0.25$, which is $> \frac{13}{72}$.

    Therefore, in this case the \MEDIAN-H\ policy is not a $\sfrac{1}{2}$-approx policy under deviation.
\end{proof}
\begin{lemma}
    \HEM-H is a $\sfrac{1}{2}$-approximation under deviation when there are only two boxes.
\end{lemma}

\begin{proof}
    Let $T = \sfrac{1}{2} \expect[X_i\sim \prior_i]{\max\{X_1, X_2\}}$. If $\priorMean_1 \ge T$, then box $1$ plays the no-information strategy $\delta(\priorMean_1)$, so the searcher's payoff is $\priorMean_1 \ge T$. 
    
    If $\priorMean_1 < T$, then box $1$ plays a binary pooling strategy with $b_1 = T$. Then since $\boxNum = 2$, from \Cref{lemma: bounding HEM}, $\priorMean_2 \ge T$. The searcher's payoff is a linear combination of $T$ and $\priorMean_2$, which is $\ge T$.
\end{proof}

\begin{lemma}
    \DP-H is a $\sfrac{1}{2}$-approximation under deviation when there are only two boxes.
\end{lemma}

\begin{proof}
    In this case, the searcher's payoff is $\max\{\priorMean_1,\priorMean_2\}$, which is $\ge \frac{\priorMean_1+\priorMean_2}{2} \ge \sfrac{1}{2} \expect[X_i\sim \prior_i]{\max\{X_1, X_2\}}$ by \Cref{lemma: bounding HEM}.
\end{proof}

\subsubsection{Multi-Box Setting}

We show that neither \DP-H nor \HEM-H are robust.

\begin{proposition}
    \DP-H is not a $\sfrac{1}{2}$-approximation under deviation.
\end{proposition}

\begin{proof}
    Consider the scenario where there are three boxes with priors $\prior_1,\prior_2,\prior_3$, such that the first box has a singular mass support on $\priorMean_1 = 0.25$ and $\prior_2,\prior_3$ are on support $\{0,1\}$ with $\priorMean_2 = \priorMean_3 = 0.2$.

    Under \DP-H, the searcher computes the threshold values for boxes $1$ and $2$ are $0.36$ and $0.2$ respectively, since these are the utilities the searcher receives from rejecting those boxes, assuming the boxes play full information. Thus box $1$ has no chance of ever getting selected because they have no mass on anything above $0.25$, and box $2$ should play the no-information strategy. The searcher under this scenario will reject any reward from box $1$ and take the reward from box $2$, with payoff $0.2$.

    We can also compute
    \begin{align*}
        \expect{\max\{X_1, X_2,X_3\}} = (1-0.2)^2 \times 0.25 + (1-(1-0.2)^2) \times 1 = 0.52
    \end{align*}
    And $0.52/2 > 0.2$, so the searcher does not achieve $\sfrac{1}{2}$-approximation.
\end{proof}

\begin{proposition}
    \HEM-H is not a $\sfrac{1}{2}$-approximation under deviation.
\end{proposition}

\begin{proof}
    Consider the scenario where there are three boxes with priors $\prior_1,\prior_2,\prior_3$, all with mean $\priorMean_1 = \priorMean_2 = \priorMean_3 = \frac{1}{3}$ and on support $\{0,1\}$.

    We can compute
    \begin{align*}
        \expect{\max\{X_1, X_2,X_3\}} = (1-\frac{1}{3})^3 \times 0 + (1-(1-\frac{1}{3})^2) \times 1 = \frac{19}{27}
    \end{align*}

    So $\frac{1}{3} = \priorMean_i \le \expect{\max\{X_1, X_2,X_3\}}/2 = \frac{19}{54}$. This means the first two boxes should deviate to binary pooling strategies setting $b_1 = b_2 = \frac{19}{54}$. The searcher's payoff under this strategy profile can be computed as 
    \begin{align*}
        \frac{18}{19} \times \frac{19}{54} + (1-\frac{18}{19}) \times \frac{1}{19} \times \frac{19}{54} + (1-\frac{18}{19})^2 \times \frac{1}{3} < \frac{19}{54}
    \end{align*}

    so that they do not achieve $\sfrac{1}{2}$-approximation.
\end{proof}



% \begin{definition}[Lower median]
%     The lower median is defined as $m = \inf\{c: \prob{\maxPrize \ge c} \le \sfrac{1}{2}\}$.
% \end{definition}

% \begin{definition}[Upper median]
%     The upper median is defined as $M = \sup\{c: \prob{\maxPrize \ge c} \ge \sfrac{1}{2}\}$.
% \end{definition}

% \begin{remark}
% There can potentially be multiple medians given the boxes' responses, as any value $v$ between $m$ and $M$ is technically considered a median. Furthermore, it is well-known that under no deviation, policies with lower medians must be strict threshold policies to be valid $1/2$-approximation policies. However, we will see in the Appendix that with deviation allowed, all variants of the median policy will result in the same Stackelberg equilibrium for the boxes' responses.
% \wt{could we move this paragraph to later sections}
% \end{remark}









==> arXiv/apx.tex <==

\label{sec:appendix}
\section{Details of Proof of \HEM\ Stackelberg Equilibrium}


\begin{proposition}
\label{prop: last box behavior}
Assume the searcher uses the \HEM\ policy in the two-box setting. For any arbitrary priors,
fixing the first box's strategy,
box $2$ is always better off by using a full information strategy.
\end{proposition}
\begin{proof}
Let us fix the first box's strategy $G_1$. 
Suppose that box $2$ chooses a strategy $G_2$
such that the resulting threshold is $\thres \equiv \HEMthreshold(G_1, G_2)$. 
Then the expected payoff of box $2$ is:
\begin{align}
    \boxU_2(G_1, G_2)
    = \prob{x_1 < \thres}
\end{align}
As we can see, whenever $G_1$
is fixed, $\boxU_2(G_1, G_2)$ is 
an increasing function with respect to the threshold $\thres$.
Thus, to maximize box $2$'s expected payoff, it suffices to 
choose to a strategy $G_2$ that maximizes the threshold $\thres$.

Notice that 
\begin{align}
    \thres 
    = \frac{1}{2}\expect[x\sim\maxPrizeCDF]{x}
    = \frac{1}{2}\expect[x\sim G_2]{\expect[x_1 \sim G_1]{\max\{x_1, x\}}}
    = \frac{1}{2}\expect[x\sim G_2]{v_2(x)}
\end{align}
where we have defined function $\interimMaxPrize_2(x) \triangleq 
\expect[x_1 \sim G_1]{\max\{x_1, x\}}$ as the expected maximum prize 
when the box $2$ realizes prize $x$. 
By the convexity of max operator, it is easy to see that this function
$\interimMaxPrize_2(x)$ is a convex function. 
Thus, when $G_2 = \prior_2$, 
we know that it maximizes $\expect[x\sim G_2]{\interimMaxPrize_2(x)}$.
\end{proof}

\begin{lemma}
\label{property of U}
We have the following properties about the function $\interimMaxPrize_1(x)$:
\begin{itemize}
    \item function $\interimMaxPrize_1$ is an increasing convex function 
    with $\interimMaxPrize_1(0)=\priorMean_2$ and $\interimMaxPrize_1(1) = 1$;
    \item the first-order derivative $\interimMaxPrize_1'(x)$ of $\interimMaxPrize_1(x)$
    satisfies $\interimMaxPrize_1'(x) \le 1$.
\end{itemize}
\end{lemma}
\begin{proof}
% \wt{placeholder ...}
By definition, we have for any $s\in [0, 1]$ and any $0 \le \delta \le (1-s)$,
\begin{align*}
    \interimMaxPrize_1(s+\delta) - \interimMaxPrize_1(s) = \int_{0}^{1} [\max\{s+\delta,x_2\} - \max\{s,x_2\}] \cdot  d \prior_2(x_2) 
    \le \int_0^1 \delta d \prior_2(x_2) = \delta
\end{align*}
Thus, $\interimMaxPrize_1'(s) = \lim_{\delta \to 0} \frac{\interimMaxPrize_1(s+\delta) - \interimMaxPrize_1(s)}{\delta} \le 1$, as desired.

\end{proof}
With the above definition, we know that 
for any strategy profile $(G, \prior_2)$
\begin{align}
    \label{alternative threshold defn}
    \HEMthreshold(G, \prior_2)
    & = \frac{1}{2} \expect[x\sim G]{\expect[x_2\sim \prior_2]{\max\{x, x_2\}}} 
    % = \frac{1}{2} \int_0^1{\int_0^1{\max(x_2, x)}}d\prior_2(x_2) dG(x)
    = \frac{1}{2} \int_0^1 \interimMaxPrize_1(x) dG(x)
\end{align}




%%% FULL INFORMATION EQUILIBRIUM STRATEGY
%%%
%%%
%%%
%%%

\begin{proposition}
\label{equilibrium case 1}
Consider a two-box setting $\boxNum = 2$, 
and arbitrary priors $\prior_1, \prior_2$. 
% but with the same mean $\priorMean_1 = \priorMean_2 \equiv \priorMean$.
If the searcher uses the \HEM\ policy and if $\priorMean_1 \ge \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$, then $(\noInfor(\priorMean_1), \prior_2)$ is one equilibrium strategy.
\end{proposition}

\begin{proof}
    Given a strategy profile $(G_1, \prior_2)$,
    the threshold used in the searcher's
    stopping strategy is $\HEMthreshold(G_1, \prior_2) = \frac{1}{2}\int_0^1 \interimMaxPrize_1(x)dG_1(x)$. 
    Notice that box $1$ always wants to 
    maximize the probability $\prob[x\sim G_1]{x \ge \HEMthreshold(G_1, \prior_2)}$. 
    Notice that function $\interimMaxPrize_1(x)$ 
    is a convex function, thus,
    $\HEMthreshold(G_1, \prior_2)$ can achieve its minimum value when $G_1$ is the No information strategy.
    Thus, when $\priorMean_1 \ge \frac{1}{2}\interimMaxPrize_1(\priorMean_1)$,
    we have $\prob[x\sim G_1]{x \ge \HEMthreshold(G_1, \prior_2)} = 1$ when $G_1$ is the No information strategy, implying that No information is indeed the best strategy for the box $1$.
\end{proof}

\noindent 
From this point forward, we assume $\priorMean_1 < \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$. 

%%% FIRST BOX BINARY SUPPORT
%%%
%%%
%%%
%%%

\begin{proposition}[Binary support suffices]
\label{binary-supp suffices}
For any priors $\prior_1$ and $\prior_2$ for boxes $1$ and $2$, if the searcher uses the \HEM\ policy, then for any box $2$'s strategy $G_2$, 
there exists a best-response strategy for box $1$ that has binary support.
\begin{proof}
Suppose that box $1$'s current strategy is $G_1$ 
and box $2$'s strategy is $G_2$, 
let $\thres \equiv \thres(G_1, G_2)$ be the threshold used by the searcher. 
% and the current threshold for box $1$'s reward to beat is $\theta = 1/2\mathbb{E}_{x \sim \max(G_1,\prior_2)}[x]$. 
In below, we show that one can construct a binary-support strategy $G_1'$
for box $1$ that always has weakly higher payoff. 
Define 
\begin{align}
a \triangleq \expect[x\sim G_1]{x \mid x< \thres},\quad
b \triangleq \expect[x\sim G_1]{x \mid x\ge \thres}
\end{align} 
Consider a binary-support strategy $G_1'$ such that $\supp(G_1') = \{a, b\}$. 
It is easy to see that strategy $G_1'$ is a valid strategy for box $1$
as we have $\prior_1 \blackwellOrder G_1 \blackwellOrder G_1'$. 
Let the threshold $\thres' \equiv \thres(G_1', G_2)$ be the threshold 
used by the searcher given the strategy profile $(G_1', G_2)$. 
Then we know $\thres' \le \thres$ as $G_1 \blackwellOrder G_1'$. 
Together with the fact that $b \ge \thres$, we have 
$\prob[x\sim G_1]{x \ge \thres} \le 
\prob[x\sim G_1']{x \ge \thres'}$.
Thus, box $1$ can always have (weakly) higher payoff by using 
strategy $G_1'$.
\end{proof}
\end{proposition}





%%% THRESHOLD STRATEGY PROOF
%%%
%%%
%%%
%%%
\begin{lemma}[Binary pooling strategy suffices]
\label{cutoff infor suffices}
Box $1$ always (weakly) prefers a binary pooling strategy. 
% If $\priorMean_1 < \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$, then 
% $(\bestResponse_1, \prior_2)$ is one equilibrium strategy
% where strategy $\bestResponse_1$ is a binary pooling strategy.
\end{lemma}
\begin{proof}
Let us fix box $1$'s strategy $G_1$ with binary support 
$\supp(G_1) = \{a, b\}$ where $0 \le a \le \priorMean_1 < b$, and 
$G_1$ has mass $p_a$ on point $a$ and mass $p_b$ on point $b$. 
Notice that we must have $b\ge \thres(G_1, \prior_2)$ otherwise 
box $1$'s expected payoff is $0$.
Suppose strategy $G_1$ is not a binary pooling strategy, 
then there must exist another strategy $G_1'$ with the support $\{a', b'\}$
such that $b ' > b$ and $p_{b'} = p_b, p_{a'} = p_a$. 
In below we now show that we always have $b' \ge \thres(G_1', \prior_2)$. 

We define a function 
\begin{align}
    f(b) 
    = \frac{1}{2}\left(p_a \interimMaxPrize_1\left(\frac{\priorMean_1 - p_b b}{p_a}\right) + p_b \interimMaxPrize_1(b)\right) - b 
\end{align}
Consider 
\begin{align*}
    f'(b) = \frac{1}{2} \left(p_a \cdot \frac{-p_b}{p_a} \interimMaxPrize_1'\left(\frac{\priorMean_1 - p_b b}{p_a}\right) 
    + p_b \interimMaxPrize_1'(b)\right) - 1
    & = 
    \frac{1}{2} \left(-p_b \interimMaxPrize_1'\left(\frac{\priorMean_1 - p_b b}{p_a}\right) 
    + p_b \interimMaxPrize_1'(b)\right) - 1  \\
    & \le 0
\end{align*}
The last inequality holds because $\interimMaxPrize_1'(b) 
\le 1$. Thus, function $f(\cdot)$ is non-increasing. 
As $b' > b$, we thus have $f(b') \le f(b) <  0$, implying that 
$b' \ge \thres(G_1', \prior_2)$.
Consequently, the expected payoff of box $1$ under 
the strategy profile $(G_1', \prior_2)$ is at least $p_b$.
This implies that binary pooling strategy is always (weakly)
better for box $1$. 
\end{proof}

%%% EXISTENCE OF EQUILIBRIA
%%%
%%%
%%%
%%%
\begin{lemma}[Property and existence of $\equilCutoff$]
\label{lem:existence of equilCutoff}
When $\priorMean_1 < \frac{1}{2} \interimMaxPrize_1(\priorMean_1)$, then 
the binary pooling strategy $\equilStrat \equiv G^{(\equilCutoff)}$
must satisfy that $b(\equilCutoff) = \HEMthreshold(\equilStrat, \prior_2)$,
and such $\equilCutoff$ always exists.

\end{lemma}
\begin{proof}
For strategy profile $(\cutoffInfor, \prior_2)$
where strategy $\cutoffInfor$ has 
$\supp(\cutoffInfor) = \{a(\cutoff), b(\cutoff)\}$,
we know that box $1$'s expected payoff is essentially 
the probability mass $1 - \prior_1(a(t))$ on the point $b(\cutoff)$. 

Thus we can formulate box $1$'s problem as follows:
\begin{align*}
    \arraycolsep=5.4pt\def\arraystretch{1}
    \tag{$\mathcal{P}(t)$}
    \label{equilibrium t}
    &\begin{array}{lll}
        \equilCutoff = \argmax\limits_{t\in [0, 1]} ~ &
        \displaystyle
        1 - \prior_1(a(t))
        \quad & \text{s.t.} 
        \vspace{1mm}
        \\
        & 
        \displaystyle
        b(t) \ge \HEMthreshold(\cutoffInfor, \prior_2). & 
    \end{array}
\end{align*}
As we can see, 
when $t = \equilCutoff$,
the constraint in the above program \Cref{equilibrium t} must be binding, namely
we have $b(\equilCutoff) = \HEMthreshold(\equilStrat, \prior_2)$. 
In below we prove the existence of $\equilCutoff$.
We consider the following function 
\begin{align*}
    f(t) 
    \triangleq \HEMthreshold(\cutoffInfor, \prior_2) - b(\cutoff)
    & = \frac{1}{2} \int_0^1 \interimMaxPrize_1(x) d\cutoffInfor(x) - b(\cutoff) \\
    & = \frac{1}{2}\cdot\left(\prior_1(\cutoff) \interimMaxPrize_1(a(\cutoff)) + 
    (1 - \prior_1(\cutoff)) \interimMaxPrize_1(b(\cutoff))\right) - b(\cutoff)
\end{align*}
Notice that $f(0) = \sfrac{1}{2}(0 + \interimMaxPrize_1(\priorMean_1)) - \priorMean_1 > 0$ and $f(1) = \sfrac{1}{2}(\interimMaxPrize_1(\priorMean_1) + 0) - 1 < 0$.
Hence by Intermediate Value Theorem, since $f$ is continuous as it is a composition of continuous functions (since $\prior_1$ is continuous by assumption), there exists $\equilCutoff$ such that $f(\equilCutoff) = 0$, as desired.

\end{proof}

%%% UNIQUENESS OF EQUILIBRIA
%%%
%%%
%%%
%%%
\begin{lemma}[Uniqueness of $\equilCutoff$]
\label{uniqueness of $\equilCutoff$}
When $\priorMean_1 < \sfrac{1}{2} \interimMaxPrize_1(\priorMean_1)$, then there exists a unique 
binary pooling strategy $\equilStrat$ such that 
$b(\equilCutoff) = \thres(\equilStrat, \prior_2)$.
\end{lemma}
\begin{proof}
We consider the following function 
\begin{align*}
    f(t) 
    = \frac{1}{2}\cdot\left(\prior_1(\cutoff) \interimMaxPrize_1(a(\cutoff)) + 
    (1 - \prior_1(\cutoff)) \interimMaxPrize_1(b(\cutoff))\right) - b(\cutoff)
\end{align*}
and consider 
\begin{align*}
    f'(t)
    & = 
    \frac{1}{2}\left( \priorPDF_1(\cutoff)\interimMaxPrize_1(a(\cutoff))+ 
    a'(\cutoff)\prior_1(\cutoff)\interimMaxPrize_1'(a(\cutoff)) 
    -  \priorPDF_1(\cutoff) \interimMaxPrize_1(b(\cutoff))
    + b'(\cutoff)(1 - \prior_1(\cutoff)) \interimMaxPrize_1'(b(\cutoff)) \right) - b'(\cutoff)
\end{align*}
We just need to show $f'(t) < 0$, where $f$ is our function above. Since $\interimMaxPrize_1$ is convex, we know that $\interimMaxPrize_1'$ is increasing, so $\interimMaxPrize_1(b(t)) \ge \interimMaxPrize_1(a(t)) + \interimMaxPrize_1'(a(t)) \cdot (b(t) - a(t))$. Hence, we just need to show 
\begin{align*}
    \frac{a'(t)\prior_1(t)\interimMaxPrize_1'(a(t)) + b'(t)(1-\prior_1(t))\interimMaxPrize_1'(b(t))}{2}
    & <
    \frac{(b(t) - a(t))\cdot \interimMaxPrize_1'(a(t)) \cdot h_1(t)}{2} + b'(t)
\end{align*}

Now, we know that 
\begin{align*}
    \prior_1(t)a(t) + (1-\prior_1(t))b(t)
    & = 
    \priorMean_1 
\end{align*}

Taking the derivative and rearranging,
\begin{align*}
    h_1(t)a(t) + \prior_1(t)a'(t) - h_1(t)b(t) + (1-\prior_1(t))b'(t)
    & = 
    0
\end{align*}
\begin{align*}
    h_1(t)(b(t)-a(t))
    & = 
    \prior_1(t)a'(t) + (1-\prior_1(t))b'(t) 
\end{align*}

Plugging this back into the original inequality, we get 
\begin{align*}
    \frac{a'(t)\prior_1(t)\interimMaxPrize_1'(a(t)) + b'(t)(1-\prior_1(t))\interimMaxPrize_1'(b(t))}{2}
    & < 
    \frac{(\prior_1(t)a'(t) + (1-\prior_1(t))b'(t)) \cdot \interimMaxPrize_1'(a(t))}{2} + b'(t)
\end{align*}

Rearranging, this becomes 
\begin{align*}
    b'(t) \cdot (1 + \frac{(1-\prior_1(t)) \cdot (\interimMaxPrize_1'(a(t)) - \interimMaxPrize_1'(b(t)))}{2})
    & \ge \frac{b'(t)}{2} >
    0
\end{align*}

as $b'(t) > 0$ and $\interimMaxPrize_1'(a(t)) - \interimMaxPrize_1'(b(t)) \ge -1$.
\end{proof}

\begin{comment}
\begin{corollary}
\label{stackelberg mean}
    The Nash Equilibrium for the two-box problem under searcher using
    \HEM\ policy is $(G_1^{*},\prior_2)$, where $G_1^{*}$ is determined by \Cref{prop: stackelberg hem}.
\end{corollary}

\begin{proof}
    We know from \Cref{prop: last box behavior} that box $2$ will always use the full-information strategy, so with this prior information, box $1$ should always use the best-response strategy to box $2$ to maximize its payoff determined by \Cref{prop: stackelberg hem}, for the Stackelberg Equilibrium.
\end{proof}
\end{comment}

\section{Details of Proof of \MEDIAN\ Stackelberg Equilibrium}

\begin{lemma}
\label{median support 2}
    Box $2$'s best response to Box $1$ can always be represented as a binary support strategy.
\end{lemma}

\begin{proof}
    Say that the current median threshold for the searcher under $\overline{G}$ is $m$ and that box $2$ switches to a binary support strategy $G_2'$ with support $\supp(G_2) = \{a_2,b_2\}$, where $a_2 = \expect[x \sim G_2]{x \mid x < m}$ and $b_2 = \expect[x \sim G_2]{x \mid x \ge m}$. We now claim under the new cdf $\overline{G'} = G_1G_2'$, the new median threshold $m'$ does not give box $1$ a higher payoff. Otherwise, we have $m' < m$ and $G_1(m') < G_1(m)$. Then
    \begin{align}
        G_2'(m') \le G_2'(m) = G_2'(a_2) \le G_2(m) \le G_2(m')
    \end{align}
    So under the new cdf,
    \begin{align}
        \overline{G'}(m) = G_1(m')G_2'(m') < G_1(m')G_2(m') < 1/2
    \end{align}
    since $m$ is the smallest median in $\overline{G}$. Thus, $m'$ cannot be the new median in $\overline{G'}$.
\end{proof}

\begin{lemma}
\label{median pooling 2}
    Box $2$'s best response to Box $1$ can always be represented as a binary pooling strategy.
\end{lemma}

\begin{proof}
    From the above proof we can let $G_2$ be box $2$'s original strategy and $G_2'$ be the binary support strategy box $2$ deviates to. Let $m$ be the \MEDIAN\ threshold for $\overline{G} = G_1G_2$ and $m'$ be the threshold for $\overline{G'} = G_1G_2'$. Then we know if $m' < a_2$, 
    \begin{align}
        \overline{G'}(a_2) = G_1(a_2)G_2'(a_2) = G_1(a_2) \cdot 0 = 0
    \end{align}
    and also 
    \begin{align}
        \overline{G'}(b_2) = G_1(b_2)G_2'(b_2) = G_1(b_2) \cdot 1 \ge G_1(m) \ge G_1(m)G_2(m) \ge 1/2
    \end{align}
    Hence $a_2 \le m' \le b_2$. Let $p_2 = \prob[x \sim G_2']{x = b_2}$, so $p_2 = \int_{m'}^1 dG_2'(x)$. Since $\int_{m'}^1 dG_2(x) \ge \int_{m'}^1 d\prior_2(x)$ and $\prior_2$ is continuous, we know there exists $m^{''} \le m'$ such that $\int_{m'}^1 dG_2(x) = \int_{m^{''}}^1 d\prior_2$. Let $G_2^{(m^{''})}$ be the binary pooling strategy with $\supp(G_2^{(m^{''})}) = \{a_2',b_2'\}$.
    
    We now show $b_2 \le b_2'$, so that $a_2' \le a_2$ and then $a_2' \le m \le b_2'$. This is because by a similar argument in \Cref{constant threshold policy multibox}, if box $2$ switches to a binary pooling strategy $G_2^{'''}$ with upper support $b_2$, then the upper support has mass $\ge p$. Thus, since the upper support of $G_2^{(m^{''})}$ has mass $p$, we know $b_2' \ge b_2$.
    
    We now claim under the new cdf $\overline{G^{''}} = G_1G_2^{''}$, the new median threshold $m^*$ does not give box $1$ a higher payoff compared to $\overline{G'}$. Otherwise, we have $m^* < m'$ and $G_1(m^*) < G_1(m')$. Then 
    \begin{align}
        G_2^{''}(m^*) \le G_2^{''}(m') = G_2^{''}(a_2') = G_2'(a_2) = G_2'(m')
    \end{align}
    So under the new cdf, 
    \begin{align}
        \overline{G^{''}}(m^*) = G_1(m^*)G_2^{''}(m^*) < G_1(m^*)G_2'(m^*) < 1/2
    \end{align}
    since $m'$ is the smallest median in $\overline{G'}$. Thus $m^*$ cannot be the new median in $\overline{G^{''}}$. 
\end{proof}

\begin{definition}
    Let $G_2^M$ be a binary pooling strategy with cutoff $m$ and support ${a(m),b(m)}$, where $m$ is the lower median of box $2$'s prior $\prior_2$. Then we define $\BM = b(m)$.
\end{definition}

We will need the definition of $\BM$ to solve the Stackelberg Equilibrium.

\begin{proposition}
\label{no info wins}
    If $\priorMean_1 \ge \BM$, then box 1 can always win with the no information strategy $\delta(\priorMean_1)$.
\end{proposition}

\begin{proof}
    Let's say box $1$ uses the no information strategy $G_1 = \delta(\priorMean_1)$. Then if box $2$ can only win if they play strategy $G_2$ such that $G_2(\priorMean_1) < 1/2$. This is because if no such strategy $G_2$ exists, then $G_2(\priorMean_1) \ge 1/2$ for all strategies $G_2$, in which case 
    \begin{align}
    \overline{G}(\priorMean_1) = G_1(\priorMean_1)G_2(\priorMean_1) \ge 1 \cdot 1/2 = 1/2    
    \end{align}
    Then box $1$ will always win if they send reward $\priorMean_1$, so box $1$ will always win. 

    We show that no such strategy $G_2$ exists. Given any arbitrary threshold $b_2$ where $b_2 > \priorMean_1 \ge \BM \ge \priorMean_2$, if box 2 wants to maximize their probability of non-strictly beating it, from \Cref{constant threshold policy multibox}, it suffices for them to use a binary pooling strategy with $b_2$ as the upper support. So box $2$'s best strategy of non-strictly beating threshold $\priorMean_1 + \epsilon$ for some $\epsilon > 0$ is a binary pooling strategy with support $\{a_2,b_2\}$ such that $b_2 = \priorMean_1 + \epsilon$. But since $\priorMean_1 \ge \BM$, we know that 
    \begin{align}
        p_{b_2} = Pr_{h \sim \prior_2}[h \ge b_2] < Pr_{h \sim \prior_2}[h \ge \BM] = 1/2
    \end{align}
    and since $a_2 < \priorMean_2 < \BM \le \priorMean_1$, $G_2(\priorMean_1) = G_2(a_2) > 1/2$. 

    In order for box $2$ to minimize the value of $G_2(\priorMean_1)$, they want to play a strategy $G_2$ that maximizes the probability of non-strictly beating the threshold $\priorMean_1$. But for all $\epsilon > 0$, we showed that for the strategy $G_2$ with the maximum probability non-strictly beating $\priorMean_1 + \epsilon$, $G_2(\priorMean_1) > 1/2$. Thus, no such strategy $G_2$ such that $G_2(\priorMean_1) < 1/2$ exists.
\end{proof}

\begin{comment}
\begin{proposition}
\label{stackelberg exists edge case}
    If $\priorMean_1 < \BM$ and $\prior_2 = \delta(\priorMean_2)$, then the Stackelberg equilibrium $(G_1^{*},\prior_2)$ consists of box $1$ using the binary pooling strategy with $b_1 = \BM$.
\end{proposition}

\begin{proof}
    If box $1$ plays a binary pooling strategy with support $\{a_1,b_1\}$ with $b_1 < \priorMean_2 = \BM$, then $\overline{G}(b_1) = G_1(b_1)G_2(b_1) = 1 \cdot 0 = 0$, so box $1$'s payoff is $0$. Otherwise, if $b_1 \ge \priorMean_2 = \BM$, then $\overline{G}(b_1) = G_1(b_1)G_2(b_1) = 1 \cdot = 1$, so box $1$ always wins if they play $b_1$. To maximize their winning probability $p_{b_1}$, they should minimize $b_1$, setting $b_1 = \BM$.
\end{proof}
\end{comment}

\begin{proposition}
\label{stackelberg exists}
    If $\priorMean_1 < \BM$, then the Stackelberg equilibrium $(G_1^{*},G_2^{*})$ consists of box $1$ using the binary pooling strategy with $b_1 = \BM$, and box $2$ using the binary pooling strategy with $b_2 = \BM$.
\end{proposition}

\begin{proof}
    Let's first consider the best response for box $2$ when box $1$ uses this strategy $G_1^{*}$, which we know can be represented as binary pooling by \Cref{median pooling 2}.

    \noindent 
    Note that when box $1$ plays $G_1^*$, they'll always win if they send reward $b_1^* = \BM$. This is because if box $2$ uses a binary pooling strategy $G_2$ with support $\{a_2,b_2\}$ and $b_2 \le b_1^*$, then 
    \begin{align}
        \overline{G}(b_1^*) = G_1^*(b_1^*)G_2(b_1^*) = G_1^*(b_1^*)G_2(b_2) = 1 \cdot 1 = 1 \ge 1/2
    \end{align}
    so $b_1^*$ exceeds the searcher's median threshold. 
    
    Otherwise, if box $2$'s binary support satisfies $b_2 > b_1^*$, then since $b_1^* \ge \BM \ge \priorMean_2 \ge a_2$, we know $p_{b_2} < 1/2$, so 
    \begin{align}
        \overline{G}(b_1^*) = G_1^*(b_1^*)G_2(b_1^*) = G_1^*(b_1^*)G_2(a_2) = 1 \cdot p_{a_2} > 1/2
    \end{align}
    so $b_1$ still exceeds the \MEDIAN\ threshold. 

    Now we show for any strategy $G_1$ that box $1$ plays, box $2$ can respond with a binary pooling strategy $G_2$ and not let box $1$ win with any reward $s_1 < \BM$. Let $G_2^*$ have support $\supp(G_2^*) = \{a_2^*,b_2^*\}$. Let $s_1^* = \arg\min_{s_1 \sim G_1} [G_1(s_1) = 1]$. If $s_1^* \ge \BM$, then box $2$ plays $G_2^*$ and for any reward $s_1 < \BM$,
    \begin{align}
        \overline{G}(s_1) = G_1(s_1)G_2(s_1) < 1 \cdot G_2(a_2^*) = 1/2
    \end{align}
    
    If $s_1^* < \BM$, then box $2$ plays $G_2 = G_2^{(\frac{s_1^*+\BM}{2})}$ with support $\supp(G_2) = \{a_2,b_2\}$ and for any reward $s_1 < \BM$,
    \begin{align}
        \overline{G}(s_1) = G_1(s_1)G_2(s_1) \le 1 \cdot G_2(a_2) < 1/2
    \end{align}
    since $a_2 < a_2^*$, so $p_{a_2} < \frac{1}{2}$.

    Hence box $1$'s goal is to maximize the probability that their reward non-strictly exceeds threshold $\BM$, since otherwise Box $2$ will play a strategy that makes the searcher reject any reward $s_1 < \BM$. From \Cref{constant threshold policy multibox}, this is $G_1^*$. There is no strategy with higher payoff for box $1$ as otherwise the searcher would accept rewards from box $1$ less than $\BM$. 
    
    Thus, $G_1^*$ is the best strategy for box $1$. Under this, $s_1^* \ge \BM$, so box $2$'s best strategy is $G_2^*$.
\end{proof}

\begin{comment}
\begin{corollary}
    There is no Nash Equilibrium for the two-box problem under searcher using \MEDIAN\ policy. \dz{Do we want to include this?}
\end{corollary}

\begin{proof}
    See the Appendix.
\end{proof}
\end{comment}

==> arXiv/neruips-apx.tex <==


The full version of this paper, including detailed proofs, can be found at \url{https://arxiv.org/pdf/2409.18269}

% \section{Missing Proofs in \texorpdfstring{\Cref{sec:opt infor}}{}}
% \label{apx:proof opt infor}
% \input{NeurIPS-24/apx-proof-opt-infor}

% \section{Missing Proofs in \texorpdfstring{\Cref{sec:general prior}}{}}
% \label{apx:proof general prior}
% \input{NeurIPS-24/apx-proof-general-prior}

% \section{Missing Proofs in \texorpdfstring{\Cref{sec:iid prior}}{}}
% \label{apx:proof iid prior}
% \input{NeurIPS-24/apx-proof-iid-prior}

% \section{Missing Proofs in \texorpdfstring{\Cref{sec:log concave}}{}}
% \label{apx:proof log concave}
% \input{NeurIPS-24/apx-proof-log-concave}
